Readout for Calorimetry at Future Colliders: A Snowmass 2021 White Paper

Calorimeters will provide critical measurements at future collider detectors. As the traditional challenge of high dynamic range, high precision, and high readout rates for signal amplitudes is compounded by increasing granularity and precision timing the readout systems will become increasingly complex. This white paper reviews the challenges and opportunities in calorimeter readout at future collider detectors.

==> IF07_WP2 (Version 1977)/futurelepton.tex <==
\subsection{FCC-ee and linear electron colliders}


%\texttt{Julia Gonski, Gabriel  Matos}
Proposed calorimeters for future $e^+e^-$ colliders span a wide variety of materials and technologies. 
These designs are motivated by physics specifications, namely to ensure that calorimeters can make precision measurements on the Higgs boson and other Standard Model (SM) particles, while providing sensitivity to beyond the SM searches. 

%Main physics goals: 
%\begin{itemize} 
%\item distinguish W/Z decays $\rightarrow$ 3/4\% dijet mass resolution $\rightarrow$ ~30\% / sqrt(E) JER (2x better than past calos) $\rightarrow$ control EM vs. non-EM responses 
%\end{itemize}

Several challenges and considerations pertain to the development of readout electronics for calorimeters in $e^+e^-$ machines.
Novel calorimeter designs such as particle flow and dual readout will require dedicated R\&D in the corresponding readout systems. 
Common to almost all new calorimeter proposals is a highly granular design, which requires a high density of readout channels and thus potentially high power consumption in a small detector area. 
The need for precise timing resolution, for example in the case of 4D calorimetry, also introduces a need for smaller feature size in ASICs and keeping pace with CMOS evolution.
Finally, the use of novel materials such as silicon and fibers introduce new challenges with cold readout or high sampling frequencies, for which there is less precedent on best practices from the LHC experiments. 
In this section, specific collider considerations and calorimeter proposals are discussed in the context of future readout system design.

\subsubsection{Readout for Linear Electron-Positron Colliders}

There are several well-developed proposals for linear electron-positron colliders, such as the International Linear Collider (ILC) or the Cool Copper Collider ($C^3$).
Several future calorimeter designs have been prepared to provide performant calorimetry in line with the physics requirements of these experiments. 
The most unique feature of these colliders from a readout perspective is the ``power pulsing" operation, wherein the beam crossing of the accelerator has a very low duty cycle (10$^{-3}$)~\cite{ILC}. 
This offers an opportunity to reduce heat load and power budget in the electronics by fast switching off during the breaks between bunch trains.
This can be especially critical in a dense calorimeter, where high channel multiplicity and small infrastructure spatial requirements mean that power consumption must be reduced to a minimum. 
Studies have been performed by the CALICE Collaboration to investigate dedicated ASIC designs that accommodate fast logic and low-noise power cycling during operation with strong spatial constraints~\cite{powerpulsing_CALICE, powerpulsing_CALICE_pflow}.

Two specific examples of calorimeter designs for future linear $e^+e^-$ colliders are the Silicon Detector (SiD) and the International Large Detector (ILD), both for the ILC. 

The SiD ECAL uses silicon as an active material, similar to that of the CMS HGCAL upgrade discussed in Section~\ref{subsec:CMS}, interleaved with tungsten absorbers.
It has excellent jet energy measurement due to a particle flow reconstruction technique that relies on fine longitudinal and transverse segmentation. 
Readout of the silicon pixels can be performed by a single chip, for example the KPiX ASIC, which is bump bonded to the sensor and reads time-over-threshold with a 2000 minimum ionizing particle (MIP) dynamic range.
The HCAL for SiD relies on scintillators read out by silicon photo-multipliers (SiPMs), which can allow for electronics to be included on-chip, providing lower operating voltages and higher speed than traditional photo-multiplier tubes.

The ILD ECAL also employs a highly granular particle flow calorimeter, but implemented via sampling of silicon diodes, or alternately through scintillator strips. 
Two options are also studied for the HCAL, based on either SiPM-on-tile technology for scintillator readout, or resistive plate chambers.
In both calorimeters, issues with signal-to-noise ratio and ghost hits in SiPM readout motivate the study of double SiPM readout for longer strips, which can maintain the stringent timing and spatial resolution requirements~\cite{ILD_SiPM}.
Prototype chip designs have been developed in the ILC context for SiPM readout~\cite{SPIROC}.

%Latency $<$ 1 BC 
%LGADs: 2101.01996
% CLIC? 

\subsubsection{Readout for Circular Electron-Positron Colliders} 

As with the ILC, future circular $e^+e^-$ colliders such as FCCee have several calorimeter proposals.
In the case of FCCee, there are two main options, the ``CLIC-Like Detector" (CLD)~\cite{CLD} and the Innovative Detector for Electron-positron Accelerator (IDEA)~\cite{IDEA} detector. 
The detector requirements are very similar to those of the ILC and the calorimeter specifications follow. 

Like all $e^+e^-$ calorimeters discussed so far, CLD uses particle flow calorimetry with the aim of reconstructing visible particle four-vectors with high precision.
It also shares much of the SiD design, in that the ECAL has a silicon-tungsten sandwich structure, and the HCAL has steel absorbers interleaved with scintillator tiles that rely on SiPM readout. The IDEA detector design differs significantly by introducing a novel copper-based dual-readout fibers calorimeter, where the elimination of longitudinal segmentation allows for finer lateral segmentation with the same number of electronic readout channels.
The fibers are read out by SiPMs, and the readout design in this scenario is driven by the challenges discussed in Section~\ref{subsec:dualreadout}.


%\subsubsection{Readout for scintillators} 
%Eg. CLD + CALICE 

%Order of magnitude fewer channels than all-silicon

%Crystals: JINST 15 (2020) P11005 [2008.00338], L3 BGO

%\subsubsection{Readout for fibers} 
%Dual (IDEA + RD52 + DREAM) 
%Low longitudinal resolution —> time stamping of energy deposits
